New Hardness Results for the Permanent Using Linear Optics

In 2011, Aaronson gave a striking proof, based on quantum linear optics, showing that the problem of computing the permanent of a matrix is #P-hard. Aaronson's proof led naturally to hardness of approximation results for the permanent, and it was arguably simpler than Valiant's seminal proof of the same fact in 1979. Nevertheless, it did not prove that computing the permanent was #P-hard for any class of matrices which was not previously known. In this paper, we present a collection of new results about matrix permanents that are derived primarily via these linear optical techniques. First, we show that the problem of computing the permanent of a real orthogonal matrix is #P-hard. Much like Aaronson's original proof, this will show that even a multiplicative approximation remains #P-hard to compute. The hardness result even translates to permanents over finite fields, where the problem of computing the permanent of an orthogonal matrix is ModpP-hard in the finite field F_{p^4} for all primes p not equal to 2 or 3. Interestingly, this characterization is tight: in fields of characteristic 2, the permanent coincides with the determinant; in fields of characteristic 3, one can efficiently compute the permanent of an orthogonal matrix by a nontrivial result of Kogan. Finally, we use more elementary arguments to prove #P-hardness for the permanent of a positive semidefinite matrix, which shows that certain probabilities of boson sampling experiments with thermal states are hard to compute exactly despite the fact that they can be efficiently sampled by a classical computer.

==> sections/finite_field_old.tex <==
%!TEX root = ../sharpie.tex

\section{Permanents over Finite Fields}
\label{sec:finite_field}

Valiant's foundational work on $\sharpP$ is well-known, but his contemporary work on the relationship between the permanent and the class we now know as $\ModkP$ is less appreciated. In another 1979 paper \cite{valiant_completeness_classes}, Valiant showed that the permanent modulo $p$ is $\ModpP$-complete, except when $p = 2$, in which case the permanent coincides with the determinant because $1 \equiv -1 \pmod{2}$. 
\begin{theorem}[Valiant \cite{valiant_completeness_classes}]
The problem of computing $\Per(M) \bmod p$ for a square matrix $M \in \mathbb F_p^{n \times n}$ is $\ModpP$-complete for any prime $p \neq 2$ (and in $\NC^2$ otherwise). 
\end{theorem}
As discussed in Appendix~\ref{sec:complexity}, $\ModpP$-hardness provides evidence for the difficulty of computing the permanent, even modulo a prime. In particular, an efficient algorithm for the problem would collapse the polynomial hierarchy. 

In the spirit of our result on real orthogonal matrices, we ask whether the permanent is still hard for orthogonal matrices in a finite field. We are not the first to consider the problem; there is the following surprising theorem of Kogan \cite{kogan:1996} in 1996. 
\begin{theorem}[Kogan \cite{kogan:1996}]
\label{thm:characteristic3easy}
Let $\mathbb F$ be any field of characteristic $3$. There is a polynomial time algorithm to compute the permanent of any \emph{orthogonal} matrix over $\mathbb F$.
\end{theorem}
In other words, for orthogonal matrices, the permanent is easy to compute for fields of characteristic 2 (since it is easy in general), but it is also easy for fields of characteristic 3 (by a much more elaborate argument)! Could it be that the permanent is easy for all finite fields of some other characteristic? No, it turns out. Using the gadgets from Section~\ref{sec:real_orthogonal}, we prove a converse to Theorem~\ref{thm:characteristic3easy}.

\begin{theorem}
\label{thm:ffmain1}
Let $p \neq 2, 3$ be a prime. There exists a finite field of characteristic $p$, namely $\mathbb F_{p^4}$, such that the permanent of an orthogonal matrix in $\mathbb F_{p^4}$ is $\ModpP$-hard.
\end{theorem}
We prove the theorem by carefully porting Theorem~\ref{thm:main_real_orthogonal} to the finite field setting. Recall that Theorem~\ref{thm:main_real_orthogonal} takes a circuit $C$ and constructs a sequence of gadgets $G_1, \ldots, G_m$ such that 
\begin{equation}
\Per(G_1 \cdots G_m) = 2^{a} 3^{b} \Delta_{C},
\label{eqn:real_orthogonal}
\end{equation}
for some $a, b \in \mathbb Z$. In general, there is no way to convert such an identity on real numbers into one over finite fields, but all of our gadgets are built out of \emph{algebraic} numbers. In particular, all of the entries are in some algebraic field extension $\mathbb Q(\alpha)$ of the rationals, where $\alpha \approx 4.182173283$ is the largest real root of irreducible polynomial
$$
f(x) = x^{16} - 40x^{14} + 572x^{12} - 3736x^{10} + 11782 x^8 - 17816 x^6 + 11324 x^4 - 1832 x^2 + 1.
$$
Each element in $\mathbb Q(\alpha)$ can be written as a polynomial (of degree less than 16) in $\alpha$ over the rationals. In Appendix~\ref{app:fftech_entries}, we give explicit canonical representations for a set of numbers which generate (via addition, subtraction and multiplication, but \emph{not} division) the entries of all our gadgets.

Each entry of a gadget $G_i$ is a polynomial in $\alpha$ with rational coefficients, so observe that we can take a common denominator for the coefficients and write the entry as an integer polynomial divided by some positive integer. By the same token, we can take a common denominator for the entries of a gadget $G_i$, and write it as $\frac{1}{k_i}\hat{G_i}$ where $\hat{G_i}$ is a matrix over $\mathbb Z[\alpha]$, and $k_i$ is a positive integer.

Now we would like to take Equation~\ref{eqn:real_orthogonal} modulo a prime $p$. In principle, we can pull $k_1, \ldots, k_m$ out of the permanent, multiply through by $Z = (k_1 \cdots k_m)^n 2^{|a|} 3^{|b|}$ to remove all fractions on both sides, and obtain an equation of the form 
$$
K \Per(\hat{G_1} \cdots \hat{G_m}) = K' \Delta_C,
$$
where $K, K'$ are integers. Then the entire equation is over $\mathbb Z[\alpha]$, so if we reduce all the coefficients modulo $p$, we get an equation over $\mathbb F_p[\alpha]$.

We show in Appendix~\ref{app:fftech_entries} that for each gadget we use, the denominator $k_i$ may have prime divisors $2$, $3$, and $23$, but no others. Hence, as long as $p \neq 2, 3, 23$ (and in the case $p = 23$, there is an alternative representation we can use, see Appendix~\ref{app:fftech}), we can divide through by $Z$, pull it back inside the permanent as the $\frac{1}{k_i}$s, and distribute each $\frac{1}{k_i}$ into the corresponding $\hat{G_i}$. This gives
$$
\Per(G_1 \cdots G_m) \equiv 2^{a} 3^{b} \Delta_{C} \pmod p,
$$
the equivalent of Equation~\ref{eqn:real_orthogonal}, but over $\mathbb F_p[\alpha]$. In particular, $G_1, \ldots, G_m$ are now orthogonal matrices in $\mathbb F_p[\alpha]$, and $\Delta_C$ has been reduced modulo $p$. 

Note that $\mathbb F_p[\alpha] \cong \mathbb F_p[x] / (f(x))$ is a ring, not a field. If $f(x)$ were irreducible modulo $p$ then it would be a field, but this will never happen for our $f$. Consider the following lemma. 
\begin{lemma}
\label{lem:squaring_roots}
Let $q$ be a prime power.  Suppose $\mathbb F_q$ is the subfield of order $q$ contained in the finite field $\mathbb F_{q^2}$. Then every element in $\mathbb F_q$ has a square root in $\mathbb F_{q^2}$. 
\end{lemma}
\begin{proof}
Let $a$ be an arbitrary element of $\mathbb F_q$. By definition, $a$ has a square root if the polynomial $f(x) := x^2 - a$ has a root. If $f$ has a root in $\mathbb F_q$ then we are done. Otherwise, $f$ is irreducible, but has a root in $\mathbb F_q[x] / \langle f(x) \rangle \cong \mathbb F_{q^2}$. 
\end{proof}
By Lemma~\ref{lem:squaring_roots}, the square roots of $2$ and $6$ are in $\mathbb F_{p^2}$, and therefore so are $2 + \sqrt{2}$ and $3 + \sqrt{6}$. Then \emph{their} square roots are in $\mathbb F_{p^4}$, so $\alpha = \sqrt{2 + \sqrt{2}} + \sqrt{3 + \sqrt{6}}$ is in $\mathbb F_{p^4}$. All the other roots of $f$ can be expressed as polynomials in $\alpha$ (see Appendix~\ref{app:fftech_galois}), so they are all in $\mathbb F_{p^4}$. Hence, the minimal polynomial of any root of $f$ (over $\mathbb F_p$) divides $x^{p^4} - x$ by a standard characterization of finite fields. It follows that $f$ factors over $\mathbb F_p$ as a product of irreducible polynomials, each of degree $1$, $2$, or $4$.

Suppose $g$ is some irreducible factor of $f$. The ideal $(g(x))$ contains $(f(x))$, so there exists a ring homomorphism $\sigma$ from $\mathbb F_p[x] / (f(x))$ to $\mathbb F_p[\alpha] / (g(x))$. Note that $\mathbb F_p[x] / (g(x))$ \emph{is} a field because $g(x)$ is irreducible over $\mathbb F_p$. Also, $\sigma$ fixes $\mathbb F_p$, so we obtain 
$$
\Per(\sigma(G_1) \cdots \sigma(G_m)) = 2^{a} 3^{b} \Delta_{C}
$$
as an equation over the field $\mathbb F_p[\alpha] / (g(x))$. For each $i$, $\sigma(G_i)$ is orthogonal in $\mathbb F_p[\alpha] / (g(x))$ as well:
$$
\sigma(G_i) \sigma(G_i)^T = \sigma(G_i G_i^T) = \sigma(I) = I.
$$
It follows that $M := \sigma(G_1) \cdots \sigma(G_m)$ is orthogonal. 

Depending on the degree of $g$, the field $\mathbb F_p[\alpha] / (g(x))$ is isomorphic to $\mathbb F_p$, $\mathbb F_{p^2}$, or $\mathbb F_{p^4}$. But $\mathbb F_{p^4}$ contains $\mathbb F_p$ and $\mathbb F_{p^2}$, so $M$ can be lifted to a matrix over $\mathbb F_{p^4}$. Given the permanent of $M$ in $\mathbb F_{p^4}$, we can easily solve for $\Delta_C$, so this completes the proof of Theorem~\ref{thm:ffmain1}. 

Theorem~\ref{thm:ffmain1} shows that for any prime $p \neq 2, 3$ there is some finite field of characteristic $p$ where computing permanents (of orthogonal matrices) is hard. In particular, $p=2$ and $p=3$ are the only cases where the permanent of an orthogonal matrix is easy to compute in \emph{every} finite field of characteristic $p$, assuming the polynomial hierarchy does not collapse. We will now show that there are primes $p$ for which this problem is hard in \emph{any} field of characteristic $p$, by showing that it is hard to compute in $\mathbb F_p$ (which is contained in every other field of characteristic $p$).   

\begin{theorem}
\label{thm:ffmain2}
For all primes $p$ that split completely in $\mathbb Q(\alpha)$, computing the permanent of an orthogonal matrix over $\mathbb F_p$ is $\ModpP$-complete. This is a sequence of primes with density $\frac{1}{16}$ beginning
$$191, 239, 241, 337, 383, 433, 673, 863, 911, 1103, 1151, 1249, 1583, 1871, 1873, 2017, \ldots$$
\end{theorem}
\begin{proof}
Recall that in the proof of Theorem~\ref{thm:ffmain1}, if $g$ is an irreducible factor of $f$, then the result applies over the field $\mathbb F_{p}[x] / (g(x)) \cong \mathbb F_{p^{\deg g}}$. We show that $g$ is degree at most $4$, but in special cases this can be improved. In particular, we want $g$ to be degree $1$ (i.e., a linear factor) for our orthogonal matrix to be over $\mathbb F_p$. 

First, observe that $\mathbb Q(\alpha)$ is a Galois extension of $\mathbb Q$. That is, every root of the minimal polynomial for $\alpha$ is in $\mathbb Q(\alpha)$. See Appendix~\ref{app:fftech_galois} for details.

We apply Chebotarev's density theorem \cite{Chebotarev}, which says that if $K$ is a finite Galois extension of $\mathbb Q$ of degree $n$, then the density of primes which split completely in $K$ is $\frac{1}{n}$. We take $K = \mathbb Q(\alpha)$, a degree 16 extension of $\mathbb Q$. 

For our purposes, a prime $p$ splits completely if and only if $f$ (the minimal polynomial for $\alpha$) factors into distinct linear terms modulo $p$. Conversely, since $\mathbb Q(\alpha)$ is a Galois extension, $f$ will split into equal degree factors. Hence, if any factor is linear, then \emph{all} the factors are linear. There are only finitely many primes which \emph{ramify}, meaning that some factor is repeated; for primes which do not ramify, there is a linear factor if and only if the prime splits completely. 

According to Chebotarev's theorem, about $1/16$ of all primes split completely and yield the desired hardness result. We verified the list of primes given in the theorem computationally. Also note that for about $3/16$ of all primes, we can prove a hardness result over $\mathbb F_{p^2}$ but not $\mathbb F_p$. 
\end{proof}

We leave open how hard it is to compute the permanent of an orthogonal matrix modulo the remaining $\frac{15}{16}$ of all primes. Other linear optical gadgets can be used for $\CSIGN$ instead of $V$, resulting in different field extensions where different primes split. For instance, there exists an orthogonal gadget for KLM's $\NS$ gate for which computing the permanent modulo $97$ is hard (see Appendix~\ref{app:ns_approach}). However, it seems impossible to design linear optical gadgets that do not involve $2$ or $3$ photons at a time, in which case writing down $\varphi(O)$ requires $\sqrt{2}$ and $\sqrt{3}$. By quadratic reciprocity, these square roots only exist if $p \equiv \pm 1 \pmod{24}$ (i.e., for about a quarter of all primes), so the remaining primes may require some other technique. 


==> sections/real_orthogonal_old.tex <==
%!TEX root = ../sharpie.tex

\section{Permanents of Real Orthogonal Matrices}
\label{sec:real_orthogonal}

The first class of matrices we consider are the real orthogonal matrices. That is, square matrices $M \in \mathbb R^{n \times n}$ with $M M^{T} = M^{T} M = I$. These matrices form a group under composition, the \emph{real orthogonal group}, usually denoted $\mathrm{O}(n,\mathbb R)$. This is a subgroup of the special unitary group, $\mathrm{U}(n, \mathbb C)$, which is itself a subgroup of the general linear group $\mathrm{GL}(n, \mathbb C)$. In other words, our hardness results will carry over to unitary matrices and invertible matrices.\footnote{See Corollary~\ref{cor:classical_groups} for a complete list of classical Lie groups for which our result generalizes.}

Our result follows the outline of Aaronson's linear optical proof that the permanent is $\sharpP$-hard \cite{aar:per}. In particular, our result depends on the KLM construction \cite{klm}, and a subsequent improvement by Knill \cite{knill:2002}, which will happen to have several important properties for our reduction. Let us briefly summarize Aaronson's argument.  Suppose we are given a classical circuit $C$, and wish to compute $\Delta_C$, the number of satisfying assignments minus the number of unsatisfying assignments.  Clearly, calculating $\Delta_C$ is a $\sharpP$-hard problem.  The first thing to notice is that there exists a simple quantum circuit $Q$ such that the amplitude $\bra{0 \cdots 0}Q\ket{0 \cdots 0}$ is proportional to $\Delta_C$. The KLM protocol \cite{klm} implies that there exists a postselected linear optical experiment simulating $Q$.  Therefore, there is some unitary $U$ implemented by a linear optical network, and Fock states $\ket{S}, \ket{T}$ such that the amplitude on $\ket{T}$ when the initial state of the system is $\ket{S}$ is proportional to $\Delta_C$.  Since this amplitude is \emph{also} proportional to to the permanent of the submatrix $U_{S,T}$ by the \ptf, computing $\Per(U_{S,T})$ allows us to calculate $\Delta_C$.

Notice that Aaronson's result does \emph{not} imply that the permanent of a unitary matrix is $\sharpP$-hard.  Indeed, it does not even prove that the permanent of an invertible matrix is $\sharpP$-hard because $U_{S,T}$ need not be invertible when $U$ is invertible.  
 
Indeed, in Aaronson's proof $\ket{S} = \ket{T} = \ket{0,1,0,1, \ldots, 0,1}$, which comes directly from the dual-rail encoding of the original KLM construction.  That is, the submatrix $U_{S,T}$ is one in which only alternating rows and columns of the original matrix $U$ are used.  Imagine instead that $\ket{S} = \ket{T} = \ket{1, \ldots, 1}$.  In this case, the matrix $U_{S,T} = U$, and the $\sharpP$-hardness of the permanent of a unitary matrix would follow.  In fact, this is \emph{exactly} what we will arrange.  Furthermore, we will be careful to use \emph{real} matrices exclusively during all gadget constructions.  This will imply that the permanent of real orthogonal matrices is $\sharpP$-hard.

In the following subsections, we will focus on the exact details of the reduction and emphasize those points where our construction differs from that of Aaronson.  

\subsection{Constructing the Quantum Circuit}
\label{subsec:quantum_circuit}
Let $C : \{0,1\}^n \rightarrow \{0,1\}$ be a classical circuit of polynomial size and let $$\Delta_C :=  \sum_{x \in \{0,1\}^n} (-1)^{C(x)}.$$  In this section, we prove the following:
\begin{theorem}
\label{thm:build_Q}
Given $C$, there exists a $p(n)$-qubit quantum circuit $Q$ such that $$\bra{0}^{\otimes p(n)} Q \ket{0}^{\otimes p(n)} = \frac{\Delta_C}{2^n}$$ where $p(n)$ is some polynomial in $n$.  Furthermore, $Q$ can be constructed in polynomial time with a polynomial number of real single-qubit gates and $\CSIGN$ gates.
\end{theorem}

Let $\O_C$ be the standard oracle instantiation of $C$ on $n+1$ qubits.  That is, suppose $\O_C \ket{x, b} = \ket{x, b \oplus C(x)}$ for all $x \in \{0,1\}^n$ and $b \in \{0,1\}$.  Let us assume we have a Toffoli gate for now and we will see how to construct it later. Since $C$ is a classical boolean function of polynomial complexity, $C$ can be implemented  \cite{toffoli} with a polynomial number of Toffoli and NOT gates\footnote{Because we require that all ancillas start in the $\ket{0}$ state, we also need the NOT gate to create $\ket{1}$ ancillas.} and a polynomial number of ancillas starting in the $\ket{0}$ state. Let us describe, briefly, one way to construct $\O_C$. 

Suppose we are given the circuit $C$ as a network of polynomially many NAND gates. For each wire, with the exception of the input wires, we create an ancilla initially in state $\ket{0}$ and use the NOT gate to put it in state $\ket{1}$. For each NAND gate (in topological ordering, i.e., such that no gate is applied before its inputs have been computed), we apply a Toffoli gate targeting the ancilla associated with the output wire, and controlled by the qubits associated with its input wires (whether they are the output of an earlier NAND gate, or an actual input). Hence, the target qubit is in state $\ket{1}$ unless both control qubits are in state $\ket{1}$, simulating a NAND gate. When we have applied all the gates, the output of the function will exist in the final register. We apply a $Z = (\begin{smallmatrix} 1 & 0 \\ 0 & -1 \end{smallmatrix})$ gate to this register, then apply the sequence of gates in reverse to uncompute the function.

% We can construct $\O_C$ using the standard method of uncomputing.  That is,
%$$\ket{x}\ket{b} \ket{0}^{q(n)} \rightarrow \ket{x}\ket{b}\ket{C(x)}\ket{\text{gar}(x)} \rightarrow \ket{x}\ket{b \oplus C(x)}\ket{C(x)}\ket{\text{gar}(x)} \rightarrow \ket{x}\ket{b \oplus C(x)} \ket{0}^{q(n)}$$
% where $q(n)$ is some polynomial in $n$ and $\text{gar}(x)$ represents the garbage bits created while computing $C(x)$.  

We can now describe the entire circuit for $Q$ (ignoring the ancilla qubits), and it is depicted in Figure~\ref{fig:quantum_circuit}.
\begin{figure}[ht]
\centering
\mbox{
\Qcircuit @C=.5em @R=.8em {
& \qw & \gate{H} & \qw & \multigate{3}{\O_C} & \qw & \gate{H} & \qw \\ 
& \qw & \gate{H} & \qw & \ghost{\O_C} & \qw & \gate{H} & \qw \\ 
&  & \raisebox{.5em}{\vdots} &  &  &  & \raisebox{.5em}{\vdots}  &  \\ 
& \qw & \gate{H} & \gate{Z} &\ghost{\O_C} & \gate{Z} & \gate{H} & \qw
}}
\caption{Circuit for $Q$, where $H$ is the standard Hadamard gate and $Z$ is the Pauli $\sigma_Z$ matrix.}
\label{fig:quantum_circuit}
\end{figure}

Then, 
$$\bra{0}^{\otimes p(n)} Q \ket{0}^{\otimes p(n)} = \frac{1}{2^n} \( \sum_{x \in \{0,1\}^n} \bra{x} \bra{-} \) \O_C \( \sum_{x \in \{0,1\}^n} \ket{x} \ket{-} \) = \frac{\Delta_C}{2^n}.$$

Recall that the KLM construction allows the conversion of any quantum circuit into a linear optical circuit \emph{provided} it is constructed from CSIGN and single-qubit gates.  Since $Q$ is constructed from Toffoli and single-qubit gates, it suffices to show how the Toffoli gate can be constructed from single-qubit gates and CSIGN gates.  Unfortunately, Aaronson's proof \cite{aar:per} uses a classic construction of the Toffoli gate which uses complex single-qubit gates (see, for example, Nielsen and Chuang \cite{nc}), which will later give rise to linear optical circuits with complex matrix representations.\footnote{Actually, the proof of Aaronson \cite{aar:per} claims that the final linear optical matrix consists entirely of real-valued entries even though the matrices of the individual single-qubit gates have complex entries.  In fact, the matrix \emph{does} have complex entries, but our construction for Toffoli suffices to fix this error.}  Therefore, we will restrict ourselves to CSIGN and \emph{real} single-qubit gates in our construction of the Toffoli gate.\footnote{Although one can argue on abstract grounds that the Toffoli gate and the set of real single-qubit gates suffice to densely generate the orthogonal matrices (i.e., $\mathrm{O}(2^n)$ for every $n>0$) \cite{shi:gate}, it will turn out to be both simpler and necessary to have an exact decomposition.  In particular, we will need an exact construction of the Toffoli gate in Section~\ref{sec:finite_field} where we discuss the computation of permanents in finite fields.}

\begin{lemma}
\label{lem:toff_proof}
There exists a circuit of CSIGN, Hadamard, and $\B$ gates which implements a Toffoli gate \emph{exactly}, where 
$$\B = \frac{1}{2}
\begin{pmatrix}
 \sqrt{2+\sqrt{2}} & -\sqrt{2-\sqrt{2}} \\
 \sqrt{2-\sqrt{2}} & \sqrt{2+\sqrt{2}} 
\end{pmatrix}.$$
\end{lemma}

We prove this lemma in Appendix~\ref{app:toff_proof}.  This completes the proof of Theorem~\ref{thm:build_Q}.


\subsection{Postselected Linear Optical Gadgets}
\label{subsec:linear_optical}

We will construct a postselected linear optical circuit $O$ which will simulate the qubit circuit $Q$ on the all zeros input via a modified version of the KLM protocol.  Importantly, we will stipulate that our linear optical experiment starts and ends with a single photon in each mode so that in the \ptf we take the permanent of $O$, not a submatrix of $O$.  Therefore, we will arrive at the following consequence\footnote{To clarify, $\ket{0 \cdots 0}$ is a tensor product of qubits in the state $\ket{0}$ and $\ket{1, \ldots, 1}$ is a Fock state with $1$ photon in every mode.}
$$\Per(O) = \bra{1, \ldots,  1} \varphi(O) \ket{1, \ldots, 1} \propto  \bra{0 \cdots 0} Q \ket{0 \cdots 0} \propto \Delta_C.$$

The first step was to convert from a classical circuit to a quantum circuit.  Below we formalize the second step: converting from a quantum circuit to a linear optical circuit.

\begin{theorem}
\label{thm:klm_plus}
Given an $n$-qubit circuit $Q$ of $\poly(n)$ CSIGN and real single-qubit gates, there exists a linear optical circuit $O$ on $4n + 2\Gamma$ modes such that 
$$\bra{1, \ldots, 1} \varphi(O) \ket{1, \ldots, 1}  = \(\frac{1}{3}\sqrt{\frac{2}{3}}\)^\Gamma \(\frac{-1}{\sqrt{6}}\)^n  \bra{0}^{\otimes n} Q \ket{0}^{\otimes n},$$
where $\Gamma$ is the number of CSIGN gates in $Q$.  Furthermore, the matrix representing $O$ is a real orthogonal matrix and can be computed in time polynomial in $n$.
\end{theorem}

We now show how to construct such a linear optical circuit $O$ using the original KLM protocol, subsequent improvements by Knill \cite{knill:2002}, and a new gadget unique to our problem.  First, let us recall our main issue with using the original KLM protocol:  to prove that \emph{orthogonal} matrices are $\sharpP$-hard, we must have that all modes start and end with exactly one photon.  There are two instances in which the original KLM protocol requires a mode to be empty at the beginning and end of the computation.  First, the $\NS$ gate postselects on the Fock state $\ket{0,1}$, and second, KLM work in a dual-rail encoding.  Therefore, half of the modes in the original KLM protocol start and end empty.

To overcome the first obstacle, we appeal to subsequent work of Knill \cite{knill:2002}, in which the $\NS$ gadget construction for CSIGN is replaced by a single $4$-mode gadget $V$, which directly implements CSIGN with two modes postselected in state $\ket{1,1}$.  The matrix for $V$ is the following:
$$V = \frac{1}{3 \sqrt{2}} \begin{pmatrix}
 -\sqrt{2} & -2 & 2 & 2 \sqrt{2} \\
 2 & -\sqrt{2} & -2 \sqrt{2} & 2 \\
 -\sqrt{6 + 2 \sqrt{6}} & \sqrt{6-2 \sqrt{6}} & -\sqrt{3+\sqrt{6}} & \sqrt{3-\sqrt{6}} \\
 -\sqrt{6-2 \sqrt{6}} & -\sqrt{6 +2 \sqrt{6}} & -\sqrt{3-\sqrt{6}} & -\sqrt{3+\sqrt{6}} \\
\end{pmatrix}
$$
from which we can calculate the exact transition amplitudes given below:
\begin{align*}
\bra{0, 0, 1, 1} \varphi(V) \ket{0, 0, 1, 1} &= \textstyle{\frac{1}{3}\sqrt{\frac{2}{3}}} & \bra{0, 1, 1, 1} \varphi(V) \ket{1, 0, 1, 1} &= 0 \\
\bra{0, 1, 1, 1} \varphi(V) \ket{0, 1, 1, 1} &= \textstyle{\frac{1}{3}\sqrt{\frac{2}{3}}} &
\bra{1, 0, 1, 1} \varphi(V) \ket{0, 1, 1, 1} &= 0 \\
\bra{1, 0, 1, 1} \varphi(V) \ket{1, 0, 1, 1} &= \textstyle{\frac{1}{3}\sqrt{\frac{2}{3}}} &
\bra{2, 0, 1, 1} \varphi(V) \ket{1, 1, 1, 1} &= 0 \\
\bra{1, 1, 1, 1} \varphi(V) \ket{1, 1, 1, 1} &= \textstyle{-\frac{1}{3}\sqrt{\frac{2}{3}}} &\bra{0, 2, 1, 1} \varphi(V) \ket{1, 1, 1, 1} &= 0
\end{align*}

We now argue that these transition amplitudes suffice to generate a postselected CSIGN.  Consider the circuit depicted in Figure~\ref{fig:app_V}.  First of all, because we postselect on the final two modes ending in the state $\ket{1,1}$, we only need to consider those transitions for which those two modes end in that state.  Secondly, because we use ``fresh'' ancillary modes for every CSIGN gate, we can always assume that those two modes start in the $\ket{1,1}$ state.  This already vastly reduces the number of cases we must consider.  Finally, we wish to know what will happen when the first two modes start in the states $\ket{0,0}, \ket{0,1}, \ket{1,0},$ and $\ket{1,1}$.  Indeed, our construction will ensure that there is never more than one photon per mode representing one of the dual-rail encoded qubits.

\begin{figure}[h]
\centering
\mbox{
\Qcircuit @C=1em @R=.6em {
\lstick{(i, 0)} & & \multigate{3}{V} & \qw & & &         & & &  \multigate{1}{\CSIGN} & \qw \\ 
\lstick{(j, 0)} & & \ghost{V} & \qw & & &           & & & \ghost{\CSIGN} & \qw \\
\lstick{\ket{1}} & & \ghost{V} & \qw & \ket{1} & & \raisebox{1em}{=} & & & \qw & \qw  \\
\lstick{\ket{1}} & & \ghost{V} & \qw & \ket{1} & &          & & &    \qw & \qw 
}}
\caption{Applying $V$ gadget to generate CSIGN.}
\label{fig:app_V}
\end{figure}

For instance, the transition amplitudes of $V$ show that whenever the modes $(i, 0)$ and $(j, 0)$ each start with a photon, there is 0 probability (after postselection) that those photons transition to a state in which one of those modes contains 2 photons and the other contains no photons.  Finally, we find that all other amplitudes behave exactly as we would expect for CSIGN.  Since each of the acceptable transitions (e.g. from the state $\ket{0,1}$ to the state $\ket{0,1}$) has equal magnitude, we only have left to check that $V$ flips the sign of the state whenever the $i$th and $j$th qubits are both in the $\ket{1}$ state.  Since this is indeed the case, $V$ implements a postselected CSIGN gate.  Importantly, because $\varphi$ is a homomorphism, we can analyze each such gate separately.  Therefore, using the above we can now construct a linear optical circuit $O$ where all of our postselected modes for CSIGN start and end in the $\ket{1}$ state. 

%$$\bra{0,1}^{\otimes n}\bra{1}^{\otimes 2\Gamma} \varphi(O) \ket{0,1}^{\otimes n}\ket{1}^{\otimes 2\Gamma}  = \(\frac{1}{3}\sqrt{\frac{2}{3}}\)^\Gamma \bra{0}^{\otimes n} Q \ket{0}^{\otimes n}.$$
We now turn our attention to the dual-rail encoding.  Instead of changing the dual-rail encoding of the KLM protocol directly, we will  start with one photon in every mode and apply a linear optical gadget to convert to a dual-rail encoding.  Of course, the number of photons in the circuit must be conserved, so we will dump these extra photons into $n$ modes separate from the modes of the dual-rail encoding.  Specifically, each logical qubit is our scheme is initially represented by four modes in the state $\ket{1,1,1,1}$.  We construct a gadget that moves a photon from the first mode to the third mode, postselecting on a single photon in the last mode.  That is, under postselection, we get the transition
$$\ket{1,1,1,1} \rightarrow \ket{0,1,2,1},$$
where the first two modes now represent a $\ket{0}$ qubit in the dual-rail encoding, the third mode stores the extra photon (which we will reclaim later), and the last qubit is necessary for postselection.  We call the gadget for this task the \emph{encoding gadget} $E$, and it is applied to the first, third, and fourth mode of the above state.  The matrix for $E$ is 
$$\encoder = \frac{1}{\sqrt{6}}
\begin{pmatrix}
 \sqrt{2} & -\sqrt{2} & \sqrt{2} \\
 0 & \sqrt{3} & \sqrt{3} \\
 -2 & -1 & 1 \\
\end{pmatrix}$$
from which we get the following transition amplitudes
\begin{center}
\begin{tabular}{l c l c l }
$\bra{1,1,1} \varphi(\encoder) \ket{1,1,1} = 0$, & & $\bra{2,0,1} \varphi(\encoder)\ket{1,1,1}  = 0$, &  & $\bra{0,2,1} \varphi(\encoder) \ket{1,1,1}= \frac{1}{\sqrt{3}}$. 
\end{tabular} 
\end{center}

After applying the encoding gadget to each logical qubit, we can implement the KLM protocol as previously discussed.\footnote{One might wonder why we cannot simply apply the encoding gadget to the \emph{entire} input, thus circumventing the need to use Knill's more complicated $V$ gadget to implement CSIGN.  Examining Theorem~\ref{thm:klm} carefully, we see that all the postselection actually happens at the end of the computation.  One might be concerned that once we measured the state $\ket{0,1}$ to implement $\NS$, those modes would remain in that state.  Nevertheless, it \emph{is} possible to compose the gadgets in such a way to allow for postselection on $\ket{0}$ while maintaining that the desired amplitude is still on the $\ket{1, \ldots, 1}$ state.  We omit such a design since $V$ will turn out to have some nice properties, including its minimal usage of ancillary modes.}  Therefore, the relevant amplitude in the computation of $Q$ is now proportional to amplitude of the Fock state which has $n$ groups of modes in the state $\ket{1,0,2,1}$ and $2\Gamma$ modes in the state $\ket{1}$.  Because we want to return to a state which has one photon in every mode, we must reverse the encoding step.\footnote{Notice that postselection was required for the encoding gadget, so it does not have a natural inverse.}  For this purpose, we construct a \emph{decoding gadget} $D$, which will not require any extra postselected modes.  We apply the gadget to the second and third modes of the logical qubit such that the two photons in the third mode split with some nonzero probability.  The matrix for $D$ is 
$$\decoder = \frac{1}{\sqrt{2}}
\begin{pmatrix}
1 & 1 \\ 1 & -1 
\end{pmatrix}$$
from which the transition condition $\bra{1,1} \varphi(\decoder) \ket{0,2} = -1/\sqrt{2}$ follows.  Nearly any two-mode linear optical gate would suffice here, but $D$, the familiar Hadamard gate, optimizes the amplitude above.  Notice that if the logical qubit had been in the $\ket{1}$ state, then we would have applied $D$ to a three-photon state.  Because of conservativity, the resulting amplitude on the $\ket{1,1}$ state would be zero.  Putting together the encoding gadget, the KLM scheme, and the decoding gadget completes the proof of the theorem.

\subsection{Main Result}
We are finally ready to prove the main result: 

\begin{theorem}
\label{thm:main_real_orthogonal}
The permanent of a real orthogonal matrix is $\sharpP$-hard.  Specifically, given a polynomially sized Boolean circuit $C$, there exist integers $a, b \in \mathbb{Z}$ and a real orthogonal matrix $O$ computable in polynomial time such that 
$$\Per(O) = 2^a 3^b \Delta_C.$$
\end{theorem}
\begin{proof}
We reduce from the problem of calculating $\Delta_C$ for some polynomially sized Boolean circuit $C$ on $n$ bits.  By Theorem~\ref{thm:build_Q}, we first construct the quantum circuit $Q$ from CSIGN and single-qubit gates such that 
$\bra{0}^{\otimes p(n)} Q \ket{0}^{\otimes p(n)} = \Delta_C/2^n$.  Let $\Gamma$ be the number of CSIGN gates in $Q$.  We then convert the qubit circuit $Q$ to a linear optical circuit $O$ on $4p(n) + 2\Gamma$ modes using Theorem~\ref{thm:klm_plus}.  Notice that we can assume without loss of generality that $p(n)$ and $\Gamma$ are both even since we can always add an extra qubit to the circuit $Q$ and/or apply an extra CISGN gate to the $\ket{00}$ state.  Combined with the fact that the output amplitudes of linear optical experiments can be described by permanents via the \ptf, we have the following chain of consequences
\begin{align*}
\Per(O) &= \bra{1, \ldots, 1} \varphi(O) \ket{1, \ldots, 1} \\
&=  \(\frac{1}{3}\sqrt{\frac{2}{3}}\)^\Gamma \(\frac{-1}{\sqrt{6}}\)^{p(n)} \bra{0}^{\otimes p(n)} Q \ket{0}^{\otimes p(n)} \\
&=  \(\frac{1}{3}\sqrt{\frac{2}{3}}\)^\Gamma \(\frac{-1}{\sqrt{6}}\)^{p(n)} \(\frac{1}{2^n}\) \Delta_C \\
&=   2^a 3^b \Delta_C,
\end{align*}
where the last equality comes from the fact that $\Gamma$ and $p(n)$ are even.
\end{proof}
 



